A Broad Comparative Evaluation of Software Debloating Tools

Software debloating tools seek to improve program security and performance by removing unnecessary code, called bloat. While many techniques have been proposed, several barriers to their adoption have emerged. Namely, debloating tools are highly specialized, making it difficult for adopters to find the right type of tool for their needs. This is further hindered by a lack of established metrics and comparative evaluations between tools. To close this information gap, we surveyed 10 years of debloating literature and several tools currently under commercial development to taxonomize knowledge about the debloating ecosystem. We then conducted a broad comparative evaluation of 10 debloating tools to determine their relative strengths and weaknesses. Our evaluation, conducted on a diverse set of 20 benchmark programs, measures tools across 12 performance, security, and correctness metrics. Our evaluation surfaces several concerning findings that contradict the prevailing narrative in the debloating literature. First, debloating tools lack the maturity required to be used on real-world software, evidenced by a slim 22% overall success rate for creating passable debloated versions of medium- and high-complexity benchmarks. Second, debloating tools struggle to produce sound and robust programs. Using our novel differential fuzzing tool, DIFFER, we discovered that only 13% of our debloating attempts produced a sound and robust debloated program. Finally, our results indicate that debloating tools typically do not improve the performance or security posture of debloated programs by a significant degree according to our evaluation metrics. We believe that our contributions in this paper will help potential adopters better understand the landscape of tools and will motivate future research and development of more capable debloating tools.

==> Tables/bench_memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\rowcolors{4}{lightgray!50}{white}
\centering
\caption{Avg. Peak Memory Performance Change}
\setlength{\tabcolsep}{6pt}
\label{tab:bench_memory}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\cline{2-4}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Benchmark Complexity}} \\ \hline
\textbf{Debloater} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline 
CHISEL & 96.7\% (7) $^{1}$ & 99.4\% (5) & 100.3\% (2) \\
CHISEL-GT & 99.6\% (7) & 99.7\% (2) & 100.4\% (1)\\
RAZOR & 98.2\% & \% 99.4(3) & 100\% (2)\\
Binary Reduce (Dynamic) & N/A & N/A & 99.9\% (1)\\ \hline
Trimmer (v2) [Agg.] & 105.1\% (6) & 109.4\% (1) & 102.9\% (2) \\
OCCAM (v2) [Agg.]  & 110.9\% & 100.9\% (1)  & N/A \\
LMCAS-SIFT [Agg.]  & 99.5\% (7) & N/A & N/A \\ \hline
Binary Reduce (Static) & 98\% (9) & 98\% (5) & N/A \\
Libfilter & 99.4\% (8) & 101.2\% (2) & N/A \\ \hline

        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item 1 \hl{need a note to indicate number of benchmarks in calc}.
      \item 2 \hl{need a note here to indicate we exclude binrec for no functioning bins}
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table*}

==> Tables/bench_runtime.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\rowcolors{4}{lightgray!50}{white}
\centering
\caption{Avg. Run Time Performance Change}
\setlength{\tabcolsep}{6pt}
\label{tab:bench_runtime}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\cline{2-4}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Benchmark Complexity}} \\ \hline
\textbf{Debloater} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline 
CHISEL & 207\% (7) $^{1,3}$ & 99.2\% (5) & 99.8\% (2) \\
CHISEL-GT & 97.6\% (7) & 100.7\% (2) & 101.8\% (1)\\
RAZOR & 102.9\% & 97.3\% (3) & 98.1\% (2)\\
Binary Reduce (Dynamic) & N/A & N/A & 100.9\% (1)\\ \hline
Trimmer (v2) [Agg.] & 110.9\% (6) & 106.1\% (1) & 129.4\% (2) \\
OCCAM (v2) [Agg.]  & 118.3\% & 104.8\% (1)  & N/A \\
LMCAS-SIFT [Agg.]  & 96.3\% (7) & N/A & N/A \\ \hline
Binary Reduce (Static) & 94.7\% (9) & 106.4\% (5) & N/A \\
Libfilter & 102.2\% (8) & 101.1\% (2) & N/A \\ \hline

        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item 1 \hl{need a note to indicate number of benchmarks in calc}.
      \item 2 \hl{need a note here to indicate we exclude binrec for no functioning bins}
      \item 3 95.4\% excluding outlier: 844.4\% performance on \texttt{gzip}
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table*}

==> Tables/expertise_maintenance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\rowcolors{2}{lightgray!50}{white}
\centering
\caption{Debloater Expertise Req. and Maintenance Difficulty}
\setlength{\tabcolsep}{6pt}
\label{tab:exp_maintenance}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Benchmark} & \textbf{Expertise} & \textbf{Maintenance} \\ \hline 
CHISEL & High & Medium  \\
CHISEL-GT & High & Medium \\
RAZOR & Medium & High  \\
BinRec-ToB  &  Medium  & High \\
Binary Reduce (Dynamic) & Medium &  High \\ \hline
Trimmer (v2) & Low & Medium \\
OCCAM (v2)  & Medium &  Medium \\
LMCAS-SIFT   & Medium* &  Medium  \\ \hline
Binary Reduce (Static)  & Low  & Low   \\
Libfilter  &  Low & Low \\ \hline
        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item * Reduces to Low for instances where automatic neck placement is successful.
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table}

==> Tables/general_specs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage\{\{table,xcdraw\}\}{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass\{\{xcolor=table\}\}{beamer}

%\begin{table*}[t]
%\rowcolors{2}{lightgray!50}{white}
%\centering
%\caption{General Debloating Specification}
%\setlength{\tabcolsep}{6pt}
%\label{tab:gen_specs}
%\resizebox{.98\textwidth}{!}{%
%\begin{tabular}{|cc|cc|cc|}

\begin{longtblr}[
  caption = {Long Title},
  label = {tab:gen_specs},
]{
  colspec = {|XX[6]|},
  rowhead = 1,
  hlines,
  row{even} = {lightgray!50},
  row{1} = {white},
}

\hline

binary&version&name&arguments&External Command sent&External client\\

bftpd&6.1&get&-D -c default-anon.conf&get myfile.txt&lftp\\ 
&&navigation&-D -c default-anon.conf&ls; cd child; ls; cd ..; ls;&\\ 
&&chmod&-D -c default-anon.conf&chmod 440 myfile.txt&\\ 
&&put&-D -c default-anon.conf&put file&\\ 
&&mkdir&-D -c default-anon.conf&mkdir second&\\ 
&&mv&-D -c default-anon.conf&mv myfile.txt myfile2.txt&\\ 
&&pwd&-D -c default-anon.conf&cd ..;cd ..;pwd;&\\
&&rm&-D -c default-anon.conf&rm myfile.txt&\\ 
&&rmdir&-D -c default-anon.conf&rmdir delete\_me&\\ 
&&rm\_disabled&-D -c disabled-cmds-anon.conf&rm myfile.txt&\\ 
&&rmdir\_disabled&-D -c disabled-cmds-anon.conf&rmdir delete\_e&\\ 
&&chmod\_disabled&-D -c disabled-cmds-anon.conf&chmod 440 myfile.txt&\\ 
&&put\_disabled&-D -c disabled-cmds-anon.conf&put file&\\ 
bzip2&1.0.5&compress via std in / std out&-c <\{\{input\}\} >\{\{output\}\}&&\\
&&decompress via std in std out&-d <\{\{input\}\} >\{\{output\}\}&&\\ 
&&force overwrite of output file&-f \{\{input\}\} \{\{output\}\}&&\\ 
&&test integrity of compressed file w/out decompression&-t \{\{input\}\} \{\{output\}\}&&\\ 
&&keep input files during compression&-k \{\{input\}\} \{\{output\}\}&&\\ 
&&help&--help&&\\
&&file doesn't exist&-c \{\{non-existent file\}\}&&\\ 
&&no args&&&\\
chown&8.2&Change ownership of a file&\{\{username\}\} \{\{file/filepath\}\}&&\\ 
&&just&-R \{\{username\}\} \{\{filepath\}\}&&\\ 
&&Change ownership of a symlink&-h  \{\{username\}\} \{\{symbolic link\}\}&&\\ 
&&error: invalid\_user&\{\{nonexistent user\}\} \{\{file\}\}&&\\ 
&&error: no\_file&\{\{username\}\} \{\{nonexistent file\}\}&&\\ 
&&help&--help&&\\ 
&&no args&&&\\
date&8.21&Display time according to parameter or format&--date '1996-1-\{\{day\}\}' +\{\{fmt\}\}&&\\ 
&&&--date '1998-1-1 3 years' +\%Y&&\\ 
&&&-d 'TZ="America/Los\_Angeles" 09:00 next Fri' && \\
&&&"-d "1997-01-19 08:17:48 +0 now" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 yesterday" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 tomorrow" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 6 years ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 7 months ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 8 weeks ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&--rfc-3339=ns -d'1970-01-01 00:00:00.2234567 UTC +961062237.987654321 sec'&&\\ 
&&&-d '2005-03-27 +1 day' '+\%Y'&&\\ 
&&&-d @-22 +\%05s&&\\ 
&&&-d @-22 +\%\_5s&&\\ 
&&&"-d "72057594037927935""&&\\ 
&&&-d 1999-12-08 +\%\_3d&&\\ 
&&&-d 1999-12-08 +\%03d&&\\ 
&&&"-d "1999-12-08 7:30" "+\%\^c""&&\\ 
&&&"--rfc-3339=ns -d "2038-01-19 03:14:07.999999999""&&\\ 
&&&--rfc-3339=sec -d @31536000&&\\ 
&&&--rfc-3339=date -d May-23-2003&&\\ 
&&&-d '1999-06-01' '+\%3004Y'&&\\ 
&&&"--utc -d '1970-01-01 UTC +961062237 sec' "+\%Y-\%m-\%d \%T""&&\\ 
&&&"--utc -d '1970-01-01 00:00:00 UTC +961062237 sec' "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-R -d "1997-01-19 08:17:48 +0""&&\\ 
&&&"-d 000909 "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-u -d '1996-11-10 0:00:00 +0' "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 4 seconds ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&-d '20050101  1 day' +\%F&&\\ 
&&&-d '20050101 +1 day' +\%F&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next second" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next minute" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next hour" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next day" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next week" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next month" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 next year" '+\%Y-\%m-\%d \%T'"&&\\ 
&&&"-u -d '08/01/97 6:00' '+\%D\&\%H:\%M'"&&\\ 
&&&"-u -d '08/01/97 6:00 UTC +4 hours' '+\%D\&\%H:\%M'"&&\\ 
&&display time for each line in a file&-u --file=\{\{filename\}\} '+\%Y-\%m-\%d \%T'&&\\ 
&&&-d '1970-01-01 00:00:01' +\%s&&\\ 
&&&-d '1970-01-01 00:00:01 UTC +2 hours' +\%s&&\\ 
&&&-d 2000-01-01 +\%s&&\\ 
&&&-d '1970-01-01 UTC 946684800 sec' +'\%Y-\%m-\%d \%T \%z'&&\\ 
&&&"-d "1997-01-19 08:17:48 this minute" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 this hour" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 this week" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 this month" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 this year" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 1 day ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 2 hours ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&&"-d "1997-01-19 08:17:48 +0 3 minutes ago" "+\%Y-\%m-\%d \%T""&&\\ 
&&error: datefile doesn't exist&-f \{\{non-existent file\}\}&&\\ 
&&help&--help&&\\ 
grep&2.19&grep with pattern on input&a input\_dir/input&&\\ 
&&-v (invert match) support\& -H (print filename) support&a -v -H -r input\_dir&&\\ 
&&-h (suppress filename output) support&1 -h -r input\_dir&&\\ 
&&-n (print line number) support&-n si input\_dir/input2&&\\ 
&&-r (recursive) support\& -l (files with match) support&1 -r input\_dir -l&&\\ 
&&-L (files without match) support&1 -r input\_dir -L&&\\ 
&&-c (count matching lines) support&randomtext -r input\_dir -c&&\\ 
&&-o (only matching) support&-o \{\{r\}\}\{\{a\}\}\{\{n\}\}\{\{d\}\}* input\_dir/input2&&\\ 
&&-q (quiet) support&1 -r input\_dir -q&&\\ 
&&-s (suppress error messages) support&1 -r input\_dir -s&&\\ 
&&&-v a input\_dir/input2&&\\ 
&&-i (ignore case) support&-i Si input\_dir/input2&&\\ 
&&-w (match whole word support&-w Si input\_dir/input2&&\\ 
&&-x (match whole line) support&-x Don\'t input\_dir/input2&&\\ 
&&-E (patterns are extended regexps) support&-E randomtext* input\_dir/input2&&\\ 
&&&'ye ' input\_dir/input&&\\ 
&&&cold input\_dir/input&&\\ 
&&&\^D input\_dir/input2&&\\ 
&&&.\$ input\_dir/input2&&\\ 
&&&\^  input\_dir/input2&&\\ 
&&&\^\$ input\_dir/input2&&\\ 
&&&\^\{\{AEIOU\}\} input\_dir/input2&&\\ 
&&&\^\{\{\^AEIOU\}\} input\_dir/input2&&\\ 
&&-F (patterns are fixed strings) support&-F randomtext* input\_dir/input2&&\\ 
&&&'not exist' input\_dir/input&&\\ 
&&&-E free\{\{\^\{\{:space:\}\}\}\}+ input\_dir/input2&&\\ 
&&&"-E "b(25\{\{0-5\}\}|2\{\{0-4\}\}\{\{0-9\}\}|\{\{01\}\}?\{\{0-9\}\}\{\{0-9\}\}?\.){3}(25\{\{0-5\}\}|2\{\{0-4\}\}\{\{0-9\}\}|\{\{01\}\}?\{\{0-9\}\}\{\{0-9\}\}?)" input\_dir/input"&&\\ 
gzip&1.2.4&compress via std in / std out&-c <\{\{input\}\} >\{\{output\}\}&&\\ 
&&decompress via std in std out&-d <\{\{input\}\} >\{\{output\}\}&&\\ 
&&force overwrite of output file&-f \{\{input\}\} \{\{output\}\}&&\\ 
&&test integrity of compressed file w/out decompression&-t \{\{input\}\} \{\{output\}\}&&\\ 
&&help&--help&&\\ 
&&error-file\_does\_not\_exist&-c \{\{nonexistent file\}\}&&\\ 
&&error-missing\_operand&-c&&\\ 
imagemagick\_convert&6.9.10-23&convert-format&input\_files/eggs.\{\{from\}\} eggs.\{\{to\}\}&&\\ 
&&resize&eggs.jpg -resize \{\{scale\}\} eggs-resized.jpg&&\\ 
&&flip&eggs.jpg -flip eggs-flipped.jpg&&\\ 
&&flop&eggs.jpg -flop eggs-flopped.jpg&&\\ 
&&negate&eggs.jpg \{\{flag\}\} eggs-negate.jpg&&\\ 
&&scale&eggs.jpg -scale \{\{scale\}\} eggs-scaled.jpg&&\\ 
&&roll&eggs.jpg -roll \{\{x\}\}\{\{y\}\} eggs-rolled.jpg&&\\ 
&&transverse&eggs.jpg -transverse eggs-transverse.jpg&&\\ 
&&transpose&eggs.jpg -transpose eggs-transposed.jpg&&\\ 
&&rotate&eggs.jpg -rotate \{\{deg\}\} eggs-transverse.jpg&&\\ 
&&crop&eggs.jpg -crop \{\{width\}\}x\{\{height\}\}\{\{x\}\}\{\{y\}\} eggs-cropped.jpg&&\\ 
lighttpd&1.4.55&get-root\_file&-D -f static-all.conf&wget http://localhost:3000/index.html&wget\\ 
&&get-nested\_file&-D -f static-all.conf&wget http://localhost:3000/dir1/file1.html&\\ 
&&get-index&-D -f static-index.conf&wget http://localhost:3000&\\ 
&&get-include\_ext&-D -f static-exclude-php.conf&wget http://localhost:3000/index.html&\\ 
&&get-exclude\_ext&-D -f static-exclude-php.conf&wget http://localhost:3000/run.php&\\ 
&&get-vhost\_1&-D -f static-vhost.conf&wget http://127.0.0.1:3000/index.html&\\ 
&&get-vhost\_2&-D -f static-vhost.conf&wget http://127.0.0.1:3000/hello.txt&\\ 
&&get-vhost\_3&-D -f static-vhost.conf&wget http://127.0.1.1:3000/hello.txt&\\ 
&&get-404&-D -f static-all.conf&wget http://localhost:3000/foo.html&\\ 
make&4.2.1&low-single\_target&file1&&\\ 
&&low-multiple\_targets&file1 file2&&\\ 
&&low-deps&file3&&\\ 
&&low-deps-update&file3&&\\ 
&&low-deps-up\_to\_date&file3&&\\ 
&&low-default\_target&&&\\ 
&&low-custom\_default\_target&&&\\ 
&&low-args\_file-stdin&-f - file1&&\\ 
&&low-args\_file&-f low-single\_target.mak file1&&\\ 
&&med\_phony&all&&\\ 
&&high-includes&file4&&\\ 
&&high-vars&install&&\\ 
&&error-invalid\_target&does\_not\_exist&&\\ 
&&error-no\_makefile&&&\\ 
&&error-file\_does\_not\_exist&-f does\_not\_exist&&\\ 
memcached&1.5.22&set\_get&&\makecell{python <<EOF \\ from memcache import Client \\ client = Client('127.0.0.1') \\ assert client.set('x'\& '10') \\ assert client.get('x') == '10' \\ EOF}&python\\ 
&&set-expiration\_get-expired&&\makecell{python <<EOF \\ import time \\ from memcache import Client \\ client = Client('127.0.0.1') \\ assert client.set('x'\& '10'\& time=2)\\ assert client.get('x') == '10'\& 'value was not set' \\ time.sleep(3.0) \\ assert client.get('x') is None\& 'value did not expire' \\ EOF}&\\ 
&&add&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.add('x'\& '10') \\
        assert client.get('x') == '10'\& 'value was not set' \\
        EOF}&\\ 
&&add\_exists&&\makecell{python <<EOF \\
        from memcache import Client\\
        client = Client('127.0.0.1')\\
        client.set('x'\& '10')\\
        assert client.add('x'\& '20') == 0\\
        assert client.get('x') == '10'\& 'value was updated'\\
        EOF}&\\ 
&&replace&&\makecell{python <<EOF \\
        from memcache import Client\\
        client = Client('127.0.0.1')\\
        assert client.add('x'\& '10')\\
        assert client.replace('x'\& '20')\\
        assert client.get('x') == '20'\& 'value was not replaced'\\
        EOF}&\\ 
&&replace\_exists&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.replace('x'\& '10') == 0 \\
        assert client.get('x') is None\& 'value was added' \\
        EOF}&\\ 
&&append&&\makecell{python <<EOF \\        from memcache import Client \\        client = Client('127.0.0.1') \\
        assert client.add('x'\& '10') \\
        assert client.append('x'\& '00') \\
        assert client.get('x') == '1000'\& 'value was not updated' \\
        EOF}&\\ 
&&append-error&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.append('x'\& '00') == 0 \\
        assert client.get('x') is None\& 'value was set' \\
        EOF}&\\ 
&&prepend&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.add('x'\& '10') \\
        assert client.prepend('x'\& '00') \\
        assert client.get('x') == '0010'\& 'value was not updated' \\
        EOF}&\\ 
&&prepend-error&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.prepend('x'\& '00') == 0 \\
        assert client.get('x') is None\& 'value was set' \\
        EOF}&\\ 
&&delete&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.add('x'\& '10') \\
        assert client.delete('x') \\
        assert client.get('x') is None\& 'value was not deleted' \\
        EOF}&\\ 
&&delete-error&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.delete('x') \\
        EOF}&\\ 
&&incr&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.set('x'\& '10') \\
        assert client.incr('x') \\
        assert client.get('x') == '11' \\
        EOF}&\\ 
&&incr-error&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.incr('x') is None \\
        assert client.get('x') is None \\
        EOF}&\\ 
&&decr&&\makecell{python <<EOF
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.set('x'\& '10') \\
        assert client.decr('x') \\
        assert client.get('x') == '9 ' \\
        EOF}&\\ 
&&decr-error&&\makecell{python <<EOF \\
        from memcache import Client \\
        client = Client('127.0.0.1') \\
        assert client.decr('x') is None \\
        assert client.get('x') is None \\
        EOF}&python\\ 
mkdir&5.2.1&Make new directory relative to local dir&\{\{dir or dirpath\}\}&&\\ 
&&make dir and parents if needed&-p \{\{dir o dirpath\}\}&&\\ 
&&make dir and set file mode&-m \{\{mode\}\} dir and dirpath&&\\ 
&&help&--help&&\\ 
&&no args&&&\\ 
nginx&&file\_server-download&"-p "\{\{trace.cwd\}\}" -c file\_server.conf"&\makecell{wget http://127.0.0.1:8080/dir1/file1.html  \\
wget http://127.0.0.1:8080/dir1/./../about.html \\
wget -O index.html http://127.0.0.1:8080}&wget\\ 
&&file\_server-404&"-p "\{\{trace.cwd\}\}" -c file\_server.conf"&wget http://127.0.0.1:8080/dir2/about.html&\\ 
objdump&2.34&flag&\{\{flag\}\} \{\{binary\}\}&&\\ 
&&flag-dyn&\{\{flag\}\} \{\{binary\}\}&&\\ 
&&flag-dyn\_static\_error&\{\{flag\}\} \{\{binary\}\}&&\\ 
&&error-file\_not\_exist&-x file\_does\_not\_exist&&\\ 
&&error-not\_obj\_file&-x /etc/passwd&&\\ 
&&error-directory&-x /home&&\\ 
pdftohtml&0.86.1&markdown&markdown.pdf&&\\ 
&&opts-range&-f 1 -l 1 markdown.pdf&&\\ 
&&opts-single\_doc&-s markdown.pdf&&\\ 
&&opts-stdout&-stdout markdown.pdf&&\\ 
&&images&BinRec.pdf&&\\ 
&&openpdf-corpus&""\{\{filename\}\}" output.html"&&\\ 
rm&8.4&"remove file& local"&\{\{file\}\}&&\\ 
&&remove directory recursive&-r \{\{dir\}\}&&\\ 
&&directory-recursive-force&-r -f \{\{dir\}\}&&\\ 
&&"remove file or directory& force"&-f \{\{file/dir\}\}&&\\ 
&&prompt before removal&-i \{\{file\}\}&&\\ 
&&help&--help&&\\ 
&&no args&&&\\ 
tar&1.14&create-multiple\_files&cf foo.tar foo bar&&\\ 
&&extract-directory\_subset&xf foo.tar -C foo ./1/10&&\\ 
&&extract-file&xf foo.tar&&\\ 
&&extract-stdin\_file&x&&\\ 
&&extract-all&-xf foo.tar&&\\ 
&&create-gzip&czf foo.tar.gz foo&&\\ 
&&extract-exclude\_file&xf foo.tar -X foo.exclude&&\\ 
&&extract-exclude\_and\_include&xf foo.tar foo bar -X foo.exclude&&\\ 
&&extract-multiple\_exclude\_files&xf foo.tar -X foo.exclude -X bar.exclude&&\\ 
&&extract-exclude\_file-path&xf foo.tar foo -X foobar.exclude&&\\ 
&&error-extract-file\_not\_in\_archive&xf foo.tar foo&&\\ 
&&error-missing-command&v&&\\ 
&&error-multiple-commands&tx&&\\ 
&&error-extract-stdout&0x&&\\ 
&&help&--help&&\\ 
&&no args&&&\\ 
uniq&8.16&stdin or filename&\{\{filename\}\}&&\\ 
&&stdin-count&-c \{\{filename\}\}&&\\ 
&&stdin-repeated&-d \{\{filename\}\}&&\\ 
&&stdin-only\_unique&-u \{\{filename\}\}&&\\ 
&&stdin-ignore\_case&-i \{\{filename\}\} &&\\ 
&&stdin-skip\_fields&-f 5 \{\{filename\}\}&&\\ 
&&stdin-skip\_chars&-s 10 \{\{filename\}\}&&\\ 
&&stdin-first\_chars&-w 10 \{\{filename\}\}&&\\ 
&&help&--help&&\\ 
&&no args&&&\\ 
wget&1.20.3&protocol-https&https://digg.com/robots.txt&&\\ 
&&protocol-http&http://echo.jsontest.com/key/value&&\\ 
&&protocol-ip&--header 'Host: echo.jsontest.com' http://\{\{'echo.jsontest.com'|gethostbyname\}\}/key/value&&\\ 
&&opts-output&-O data.json http://echo.jsontest.com/key/value/key2/value2&&\\ 
&&opts-timeout\_expired&-T 10 http://echoss.jsontest.com/&&\\ 
&&opts-timeout\_ok&-T 2 http://echoss.jsontest.com/&&\\ 
&&get-param&-O data.json http://md5.jsontest.com/?text=hello\_world&&\\ 
nmap&7.93&tcp-port-scan&-sT 127.0.0.1&&\\ 
&&tcp-port scan range&"-sT -p1-7080&8080 127.0.0.1"&&\\ 
&&service scan&-sT -sV 127.0.0.1&&\\ 
&&service scan output&-sT -sV -oG report 127.0.0.1&&\\ 
&&service scan output&-sT -sV -oN report 127.0.0.1&&\\ 
&&service scan output&-sT -sV -oX report 127.0.0.1&&\\ 
sort&8.16&help&--help&&\\ 
&&no args&<no args>&&\\ 
&&reverse sort&-r <file>&&\\ 
&&stabilize sort&-s <file>&&\\ 
&&unique sort&-u <file&&\\ 
&&zero terminate lines&-z <file>&&\\

\end{longtblr}
%\end{tabular}%
%}
%\vspace{-.5em}
%\end{table*}

==> Tables/spec_generation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\rowcolors{4}{lightgray!50}{white}
\centering
\caption{Avg. Time (minutes) to Create Specification}
\setlength{\tabcolsep}{6pt}
\label{tab:spec_gen}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\cline{2-4}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Benchmark Complexity}} \\ \hline
\textbf{Debloater} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline 
CHISEL & N/A* & 403  & 180  \\
CHISEL-GT  & 30 & 403 & 180 \\
RAZOR & 30 & 42  & 35  \\
BinRec-ToB  & 19 & 49  & 36  \\
Binary Reduce (Dynamic)  & 30 & 42  & 35  \\
Trimmer (v2) [Agg.] & 3 & 5  & 10  \\
OCCAM (v2) [Agg.]  & 3 & 5  & 45  \\
LMCAS-SIFT [Agg.]  & 19 &  6 &  11 \\ \hline

        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item * Specifications available as part of CHISELBench\cite{chiselbench}.
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table}

==> Tables/tool_memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\rowcolors{4}{lightgray!50}{white}
\centering
\caption{Avg. Peak Memory (MB) per Debloater}
\setlength{\tabcolsep}{6pt}
\label{tab:tools_mem}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\cline{2-4}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Benchmark Complexity}} \\ \hline
\textbf{Debloater} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline 
CHISEL & 306 (9) & 91 (5)  & \hl{?}  \\
CHISEL-GT  & 2145 (9) & 1675 (4) & \hl{?} \\
RAZOR & 32  & 60 (5)& 31875 \\
BinRec-ToB  & 1236 (9)  & 1248 (3)  &  1231 (4)  \\
Binary Reduce (Dyn.) & 456 & 853 & 1085  \\ \hline
Trimmer (v2) [Agg.] & 3440 &  6518 & 5259  \\
OCCAM (v2) [Agg.]  & 73 & 5565  & 147 \\
LMCAS-SIFT [Agg.]  & 456 & 660 (5) & 2001 (1) \\ \hline
Binary Reduce (Static) & 415 & 1577 & 3010 \\
Libfilter & 303 & 503 & 465 \\ \hline

        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item 1 \hl{need a note to indicate number of benchmarks in calc}.
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table}

==> Tables/tool_runtime.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\rowcolors{4}{lightgray!50}{white}
\centering
\caption{Avg. Time (CPU minutes) to Run Debloater}
\setlength{\tabcolsep}{6pt}
\label{tab:tools_runtime}
%\resizebox{.98\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\cline{2-4}
 \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Benchmark Complexity}} \\ \hline
\textbf{Debloater} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline 
CHISEL & 282 (9)$^1$ & 15 $^2$  & \hl{?}  \\
CHISEL-GT  & 4078 (9) & 4058 (6) & \hl{?} \\
RAZOR & <1  & 1 (5) & 18 \\
BinRec-ToB  & 2 (9) & 3 (3)  &  3 (3)  \\
Binary Reduce (Dyn.) & 1 & 3 &  3 \\ \hline
Trimmer (v2) [Agg.] & 2 & <1 $^2$  &  18 \\
OCCAM (v2) [Agg.]  & <1 & <1 $^2$  &  <1 \\
LMCAS-SIFT [Agg.]  & <1 & <1 (4)  & 5 (1) \\ \hline
Binary Reduce (Static) & 1 & 9 & 20 \\
Libfilter & <1 & <1 & <1 (2) \\ \hline

        
\end{tabular}%
\begin{tablenotes}
      %\scriptsize
      \item 1 \hl{need a note to indicate number of benchmarks in calc}.
      \item 2 \hl{need a note to indicate near outlier failures removed?}
    \end{tablenotes}
\end{threeparttable}
%}
\vspace{-.5em}
\end{table}
